Learning Robust Controllers Via Probabilistic Model-Based Policy Search

Model-based Reinforcement Learning estimates the true environment through a world model in order to approximate the optimal policy. This family of algorithms usually benefits from better sample efficiency than their model-free counterparts. We investigate whether controllers learned in such a way are robust and able to generalize under small perturbations of the environment. Our work is inspired by the PILCO algorithm, a method for probabilistic policy search. We show that enforcing a lower bound to the likelihood noise in the Gaussian Process dynamics model regularizes the policy updates and yields more robust controllers. We demonstrate the empirical benefits of our method in a simulation benchmark.

==> Apppendix/pilco_proof.tex <==
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
%\theoremstyle{definition}
\newtheorem{dfn}{Definition}
\newtheorem{assum}{Assumption}

\newcommand{\bigo}{\mathcal{O}}


\begin{algorithm}[H]
%\SetAlgoAligned
\KwIn{$\hat{f}$, parametric policy $\pi_\theta$}

Initialize randomly $\theta_0$ \hfill \# Send random signals to the system 

Collect $N_{init}$ samples trajectories in $\mathcal{D}$ 

k=1

\While{Not \textit{Termination criterion}}{
    Train $\hat{f}_{k}$ on $\mathcal{D}$
    
    Find $\theta_{k} ~=~\text{argmin } \widehat{V_{\theta_{k-1}}}(x^0)$ 
    
    Collect trajectory $\tau$ \hfill \# rollout $\pi_{\theta_k}$ in the environment
    
    $\mathcal{D}_k = \mathcal{D}_{k-1} \cup \{\tau\}$ \hfill \#Concatenate the new trajectory 
    
    k = k + 1
}
\KwOut{$\pi_{\theta^*}$}
\caption{PILCO}
\label{algo:PILCO}
\end{algorithm}
\vspace{0.5cm}

Let's write the closed-loop dynamics as $f_\theta(\cdot | x ) := f(\cdot |x, \pi_\theta(x))$

\begin{dfn}[Value functions]
\begin{equation}
    V_\theta(x^0) = 
    \mathbb{E} \left[ \sum_{t=0}^T c(x_t) | f_\theta \right]
\end{equation}
and the one given approximate dynamics

\begin{equation}
    \widehat{V_\theta}(x^0) = 
    \mathbb{E} \left[ \sum_{t=0}^T c(x_t) | \hat{f_\theta} \right]
\end{equation}
\end{dfn}

\begin{dfn}[Sufficiently accurate model]

A sequence of models $\left\{ \hat{f}_k \right\}_{k}$ is  p-probabilistically sufficiently accurate if the following condition holds 

\begin{equation}
\label{eq:sufficiently_accurate}
    P\left(I_k = 1 | \mathcal{F}_{k}\right) \geq p 
\end{equation}

where $\mathcal{F}_{k}$ is the natural filtration generated by the closed-loop dynamics $\hat{f}_{\theta_i},~ i=0 \dots k$
and $I_k = \mathbf{1} \left\{ KL(f_{\theta_k} \| \hat{f}_{\theta_k} )< \epsilon \right\}$ for an arbitrary $\epsilon > 0$
\end{dfn}
%model accurate "in probability": weaker assumption than almost surely

\begin{lem}[Error bound on value functions]
The difference between true and approximate value function is bounded by the KL divergence between the exact and approximate dynamics.

\begin{equation}
    \left| V_\theta(x^0) - \widehat{V}_\theta(x^0)\right|  = \bigo \left(T \times KL(f_\theta \| \hat{f}_\theta)  \right)
\end{equation}
\end{lem}
\label{lem:value_fns__bound}

\begin{proof}\todo{rewrite that}
\todo{check assumptions. In practice, we only need the gradients to be in the same directions with high probability, so the bound does not need to be tight}
%Done on paper need to write it up here:write distribution over a whole trajectory. Difference between distribution in true and approximate dynamics is upper bounded by $T ~ \times KL$

Let's write a trajectory as $\xi = \left\{(x_0, u_0) \dots (x_T, u_T) \right\}$
The distribution of the trajectory is
$P(\xi) = P_0(x_0) \prod_{t=0}^{T-1} \pi_\theta(x_t) f(x_{t+1}|x_t, u_t)$

Using $log(P(\xi)) - log(\widehat{P(\xi)})= \sum_{t=0}^{T-1} log\left(\dfrac{f(x_{t+1}|x_t)}{\hat f(x_{t+1}|x_t)}\right)$ we derive

\begin{equation}
\begin{aligned}
    KL\left(P \| \hat{P} \right) = & \int P(\xi) log \dfrac{P(\xi)}{\hat{P}(\xi)}d\xi \\
    %&= \int P(x_0, \dots, x_T) \sum_{t=0}^{T-1} log\left(\dfrac{f(x_{k+1}|x_k)}{\hat f(x_{k+1}|x_k)} \right)dx_0\dots dx_{T-1}
    & =  P(x_0) \sum_{t=0}^{T-1} \prod_{k \neq t}\pi(x_k)f(x_{k+1}|x_k) 
    \int \pi(x_t)f(x_{t+1}|x_t) log\left(\dfrac{f(x_{t+1}|x_t)}{\hat f(x_{t+1}|x_t)}\right)d\xi \\
    & \leq \|\pi\|_{\infty}^{T-1} \|f\|_{\infty}^{T-1}\times T \times KL\left(f \| \hat f \right)\\
    & = \bigo \left(T \times KL\left(f \| \hat f \right) \right)
\end{aligned}
\end{equation}

%We conclude, by noting that the value function can be written as  $V(x^0) = \int C(\xi)dP(\xi)$
\todo{problem here to conclude, maybe total divergence is more suited}
\end{proof}


The consequence of lemma \ref{lem:value_fns__bound} is that if we have access to a function $\hat{f}$ which is very close to $f$ we can recover a good estimate of the value function.

%Can we ensure $\hat{f}$ becomes as close as possible to $f$? $\rightarrow$ system id° problem, since data to train the model is gathered in closed-loop


\begin{lem}[Convergence of approximate dynamics]
The sequence of $\hat{f}_k$ converges towards the exact dynamics with probability $p$.
\label{lem:iterations_bound}
\end{lem}

\begin{proof}
The sequence of KL divergence is monotonically decreasing \textbf{because we're considering the closed-loop dynamics}\todo{verify that assertion}
\begin{equation}
    KL \left(f_{\theta_{k-1}} \| \hat{f}_{\theta_{k-1}} | \mathcal{D}_k \right) \leq 
    KL\left(f_{\theta_{k-1}} \| \hat{f}_{\theta_{k-1}} | \mathcal{D}_{k-1}\right)
\end{equation}
Because the KL is lower-bounded by 0, the stopping time 
%todo consider using Hoeffding inequality (Recht book p110)

$N_\epsilon = \text{min}\left\{k \in \mathbb{N},~ P(I_k=1 | \mathcal{F}_k) > p \right\}$ 
is well defined (ie $\mathbb{E}\left[N_\epsilon\right] < +\infty$)
% is $N_\epsilon = \text{min}\left\{k \in \mathbb{N},~ I_k=1  \right\}$ sufficient?
\end{proof}
\todo{is it possible to derive an analytical bound for $\mathbb{E}[N_\epsilon]$?}


\begin{thm}
Under assumptions \todo{TODO}, PILCO converges
\begin{equation}
    \theta_k  \rightarrow \theta^*  
\end{equation}
\todo{what type of convergence, narrow, in proba or a.s.?}
\end{thm}

\begin{proof}
\todo{TODO: using previous lemmas and eq (\ref{lem:value_fns__bound})}, the stopping time 
$N_\delta = \text{min}\left\{k \in \mathbb{N},~ |V_{\theta_k} - \widehat{V_{\theta_k}}| < \delta \right\}$ is well defined. \todo{analytical bound for $\mathbb{E}[N_\delta]$ as a function of $N_\epsilon and p$}
% bounds as a function of (1/(1-2p))[...]
\end{proof}







==> Methods/methods_v0.tex <==
\subsection*{The PILCO Framework}
We consider the Markov Decision Process $(\mathcal{X, U}, f, C, T)$, representing respectively continuous state and action spaces, transition kernel, cost function and episode length. We define the cost-to-go as $\mathcal{G}_{\theta}(x) = \sum_{t=1}^{T} C(x_t, a_t) | x_0=x, \pi_\theta$, is the sum of local cost obtained when starting at $x_0$ applying the policy $\pi_{\theta}$. The expected value of this random variable is known as the value function, which is to be minimized to solve the problem:

\begin{equation}
    \theta^* = \underset{\theta}{\text{argmin}}~ V_{\theta}(x^0) =  \underset{\theta}{\text{argmin}} ~ \mathbb{E}\lbrack \mathcal{G}_{\theta}(x^0) \rbrack
\end{equation}
\label{eq:objective_return}


The PILCO algorithm \cite{Deisenroth2011} is comprised of an estimate $\hat{f}(\cdot | x_t,u_t)$ of the transition kernel and a parametric policy $\pi(\cdot | x_t, \theta)$. $\hat{f}$ is trained to predict one-step ahead prediction via empirical risk minimization on the collected data $\lbrace (x_i, u_i), x_i'\rbrace)_{i=1 \dots N}$ and $\pi$ minimizes the cost on predicted trajectories.

To do so, we need to compute the distribution of the trajectory given current policy and model. The next-state distribution is given by $p(x_{t+1} = \int \hat{f}(x_t, u_t)p(s_t, u_t) dx du$ for $t=1 \dots T$ and $x_0$ sampled from an initial distribution $\mathcal{P}_0$. Because this integral is intractable, some form of approximation is required. This can be done via Moment Matching, Bayesian quadrature or Monte-Carlo sampling. \todo{references}

The policy is then optimized given the surrogate cost-to-go
\begin{equation}
\label{eq:surr_return}
\begin{aligned}
&\theta^* = \underset{\theta}{\text{argmin}}~  V_{\theta, \hat{f}}(x^0) =  
    \mathbb{E} [ \sum_{t=1}^T C(x_t, u_t) ] \\
& \text{where } x_{t+1} \sim \hat{f}(x_t, u_t),~u_t \sim \pi_{\theta}(x_t)
\end{aligned}
\end{equation}
%where $x_{t+1} \sim \hat{f}(x_t, u_t)$ and $u_t \sim \pi_{\theta}(x_t)$

%TODO write pseudo code
As we see in the objective \ref{eq:surr_return}, the local costs are integrated over all the plausible trajectories. This means all the values between the optimistic and pessimistic returns are weighted by their relative probability. As a consequence, it does account for the worst-case and optimizes for it. We believe this trait causes the learned controllers to be robust to environmental perturbations, even if they are not explicitly present in the training phase.


\subsection*{Learning With Constraints}
%no discount factor for risk-averse MDP
In many real-world scenarios, constraints are required to guarantee the safety of the agent. We follow the formulation from \cite{Chow2018} and augment the MDP with a constraint cost function $D(x, u)$.  In the following, we omit the dependence on $\hat{f}$ for clarity.

Similarly to previous section, we define the \textit{risk-to-go} as
$\mathcal{G}_\theta(x) = \sum_{t=1}^T D(x_t, u_t | x_0=x, \pi_\theta$

We can then write the full objective

\begin{equation}
    \begin{aligned}
    \label{eq:full_objective}
     %\underset{\theta}{\textit{min}}
     \min_\theta~&V_\theta(x^0) \\ 
     \text{ subject to }  &\mathbb{E} \left[ \mathcal{G}_\theta(x^0) \right] < \beta
    \end{aligned}
\end{equation}

\begin{comment}
For a random variable $Z$ representing that cost, we write the \textit{conditional value-at-risk} as 
\begin{equation}
\begin{aligned}
    \text{CVaR}_\alpha(Z) = \underset{\nu \in \mathbb{R}}{min} 
    \left\{ \nu + \dfrac{1}{1-\alpha} \mathbb{E}\left[ (Z - \nu)^+ \right]   \right\}
\end{aligned}
\end{equation}

The \textit{CVaR-constrained} optimisation problem can then be written as

\begin{equation}
    \underset{\theta}{\text{min}}~ V_\theta(x^0) & \text{ subject to } 
    & \text{CVaR}_\alpha(\mathcal{J}_\theta(x^0) \leq \beta
\end{equation}
\label{eq:objective_return_constrained}

Which is equivalent to
\begin{equation}
    \underset{\theta, \nu}{\text{min}}~ V_\theta(x^0) & \text{ subject to } 
    & H_\alpha (\mathcal{J}_\theta(x^0), \nu ) \leq \beta
\end{equation}
\label{eq:objective_return_constrained_H}
\todo{write surrogate cost/risks?}

Where $H_\alpha(Z, \nu) = \nu + \dfrac{1}{1-\alpha} \mathcal{E} \left[ (Z-\nu)^+ \right]$. \todo{explain benefits of CVaR}
\end{comment}



Lagrangian relaxation
\begin{equation}
    \underset{\lambda \geq 0}{\text{max}}~\underset{\theta}{\text{min}} \left\{
    L(\nu, \theta, \lambda) = V_\theta(x^0) + \lambda 
    \left(\mathbb{E} \left[\mathcal{G}_\theta(x^0)\right] - \beta \right)
    \right\}
\end{equation}
\label{eq:lagrangian_full}


\subsubsection*{Heuristic based multiplier updates}
Following the algorithm described in \cite{Polymenakos2017}, algorithm 1
We define $Q_\theta(x^0) = \left(\mathbb{E} \left[\mathcal{G}_\theta(x^0)\right] - \beta \right)$

At each episode, the multiplier is updated as follow:
\begin{itemize}
    \item if $Q > \epsilon$: increase $\lambda$ is $Q > \text{upper threshold}$
    \item else decrease $\lambda$
\end{itemize}
In the original formulation, it is done in the opposite way as $Q$ defined probability of occupation in safe sets.

\begin{comment}
In contract, CPO  \cite{Achiam2017}, solves for the optimal $\lambda$ at each iteration before updating $\theta$ which incurs an inner-loop optimisation procedure

\end{comment}

\subsubsection*{Primal-Dual Method}
as in \cite{Chow2018, Chow2014}, we iteratively ascend the Lagrangian in $\lambda$, and descend along $\theta$. % and $\nu$
%TODO interpretation: if risk-to-go is low, reduce the multiplier to encourage maximising the rewards



\begin{equation}
\begin{cases}
\nabla_\theta L(\theta, \lambda)= \nabla V_\theta + \lambda \nabla Q_\theta \\
\partial_\lambda L(\theta, \lambda) = Q_\theta\\
\end{cases}
\end{equation}



It is worth noting that the update in $\lambda$ is very similar to the heuristic previously defined. \todo{then what are benefits?}




%improvement on previous methods ? 
% SGD on controller loss with initial state sampled from memory buffer, enables shorter rollouts + escape local minima in \theta  : works in practice
% theoretical guarantee for constraint satisfactions?
% can we show performance not degraded if slight changes in eval environment
